Convergence of diffusions and their discretizations: from continuous to discrete processes and back

In this paper, we establish new quantitative convergence bounds for a class of functional autoregressive models in weighted total variation metrics. To derive our results, we show that under mild assumptions, explicit minorization and Foster-Lyapunov drift conditions hold. The main applications and consequences of the bounds we obtain concern the geometric convergence of Euler-Maruyama discretizations of diffusions with identity covariance matrix. Second, as a corollary, we provide a new approach to establish quantitative convergence of these diffusion processes by applying our conclusions in the discrete-time setting to a well-suited sequence of discretizations whose associated stepsizes decrease towards zero.

==> V_norm_continuous_continuous_drift.tex <==
Note that if \Cref{ass:item:diff_disc}-\ref{item:equality_inside} holds then $\Rker_{\gamma, n}$ is nothing more than the projected Euler-Maruyama discretization of the continuous \SDE \ given by \eqref{eq:diff}.
We are now ready to state the following minorization condition on the integrated continuous kernel $\Pker_1$.
\begin{proposition}
\label{prop:doeb_continuous}
  Assume \tup{\Cref{as:item:lip}-\ref{assum:b_min}($\mtt, \rset^d$)}, \tup{\Cref{ass:loc_lip_b}}, \tup{\Cref{ass:item:diff_disc}} and
\tup{\Cref{assum:unif_integr}}. Then for any $\ell \in \nsets$ and $x,y \in \rset^d$,
\begin{equation}
  \tvnorm{\updelta_x \Pker_{\ell} - \updelta_y \Pker_{\ell}}   \leq 1 - 2\Phibf(-\alpha_{\continuous}(\mtt, \ell)^{-1/2} \|x-y\|/2) \eqsp,
\end{equation}
where
\begin{equation}
  \label{eq:def_alpha_cont}
  \alpha_{\continuous}(\mtt, \ell) =
  \begin{cases}
    (1 - \exp(-2\mtt \ell))/(2\mtt) &\text{if } \mtt \neq 0 \eqsp ; \\
    \ell &\text{ otherwise} \eqsp .
    \end{cases}
\end{equation}
\end{proposition}

\begin{proof}
  We can apply \Cref{prop:general_bound}, with $W = 1$ and $\ell \in \nsets$. We obtain that for any $x,y \in \rset^d$
  \begin{equation}
    \tvnorm{\updelta_x \Pker_{\ell} - \updelta_y \Pker_{\ell}} \leq \limsup_{m \to +\infty} \tvnorm{\updelta_x \Rker_{1/m, n}^{m\ell}- \updelta_y \Rker_{1/m, n}^{m\ell}} \eqsp .
  \end{equation}
  Let $x,y \in \rset^d$.
  In addition, let $n \in \nset$ such that $x,y \in \cball{0}{n}$ and $m \in \nsets$ with $m \geq m_0$ where $m_0 > \Lip_n^2 / (2 \mtt)$ if $\mtt < 0$ and $m_0 = 0$ otherwise.
  We consider the Markov chain associated with $\Rker_{1/m,n}$. Note that using \Cref{ass:item:diff_disc}-\ref{item:equality_inside} we have that $\Rker_{1/m, n}$ is given by \eqref{eq:kernel_langevin} with $\Tg(x) = x + \gamma b(x)$ and $\Pi = \Pi_{\msk_n}$.
  It is clear that \Cref{ass:non_expansive_Pi} holds since $\Pi_{\msk_n}$ is non-expansive. Further, we have that for any $x,y \in \cball{0}{n}$, $\gamma \leq 1/m_0$
  \begin{equation}
    \norm{\Tg(x) - \Tg(y)}^2 \leq (1 + \gamma \kappa(\gamma)) \norm{x-y}^2 \eqsp ,
  \end{equation}
with $\kappa(\gamma) = -2\mtt + \gamma \Lip_n^2$. We have that for any $\gamma \in \ocint{0, 1/m_0}$, $\kappa(\gamma) < 0$ if $\mtt >0$ and $\kappa(\gamma) \geq 0$ otherwise. Note that for any $m \geq m_0$, $\kappa(1/m) \neq 0$. We distinguish three cases:
\begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]
\item In the case where $\mtt >0$, \Cref{assum:lip_op}-\ref{assum:lip_op_str_convex} is satisfied with $\bgamma = 1/m_0$. Applying \Cref{theo:minorization_general} with $\msa = \msx$ and \eqref{eq:Xi_equality} in \Cref{lemma:technical_doeb_0} we obtain that
  \begin{multline}
    \tvnorm{\updelta_x \Rker_{1/m,n}^{m\ell}- \updelta_y \Rker_{1/m,n}^{m\ell}} \leq \probaMarkov{}{X_{m\ell} \neq Y_{m\ell}} \\ \leq 1 -  2 \Phibf\parenthese{- (- \kappa^{-1}(1/m) \defEns{ \exp\parentheseDeux{-\ell m \log \defEns{1 +  \kappa(1/m)/m}} -1})^{-1/2} \| x- y \|/2 } \eqsp . \label{eq:ineq_1}
  \end{multline}
  Therefore using that $\kappa(\gamma) = -2\mtt + \gamma \Lip_n^2 < 0$ for any $\gamma \leq 1/m_0$ and taking the limit $m \to +\infty$ in \eqref{eq:ineq_1}, we obtain that
  \begin{equation}
    \tvnorm{\updelta_x \Rker_{1/m,n}^{m\ell}- \updelta_y \Rker_{1/m,n}^{m\ell}} \leq 1 - 2\Phibf \parenthese{\alpha_{\continuous}(\mtt, \ell)^{-1/2}\norm{x-y}/2} \eqsp . \label{eq:goal}
  \end{equation}
  
\item In the case $\mtt < 0$, \Cref{assum:lip_op}-\ref{assum:lip_op_non_convex} is satisfied with $\bgamma = 1/m_0$. Applying \Cref{theo:minorization_general} with $\msa = \msx$ and \eqref{eq:Xi_equality} in \Cref{lemma:technical_doeb_0} we obtain that \eqref{eq:goal} holds taking $m \to +\infty$.
\item In the case $\mtt = 0$, \Cref{assum:lip_op}-\ref{assum:lip_op_non_convex} is satisfied with $\bgamma = 1/m_0$. Again, applying \Cref{theo:minorization_general} with $\msa = \msx$ and \eqref{eq:Xi_equality} in \Cref{lemma:technical_doeb_0} we get that
  \begin{multline}
    \tvnorm{\updelta_x \Rker_{1/m,n}^{m\ell}- \updelta_y \Rker_{1/m,n}^{m\ell}} \\ \leq 1 -  2 \Phibf\parenthese{- (- \kappa^{-1}(1/m) \defEns{ \exp\parentheseDeux{-\ell m \log \defEns{1 +  \kappa(1/m)/m}} -1})^{-1/2} \| x- y \|/2 }\eqsp ,
  \end{multline}
with $\kappa(\gamma) = \gamma \Lip_n^2$. Therefore taking $m \to +\infty$ we obtain
\begin{equation}
  \tvnorm{\updelta_x \Rker_{1/m,n}^{m\ell}- \updelta_y \Rker_{1/m,n}^{m\ell}} \leq 1 -  2 \Phibf\parenthese{-\ell^{-1/2}\norm{x-y}/2} \eqsp ,
\end{equation}
which concludes the proof.
\end{enumerate}

\end{proof}


% \begin{proof}
%     First we have for any $\ x,y \in \rset^d$, $M \geq 0$ and $n \in \nsets$ with $n^{-1} < \bgamma$
%   \begin{equation}
%     \tvnorm{\updelta_x P_1 - \updelta_y P_1} \leq  \tvnorm{\updelta_x P_1 - \updelta_x R_{1/n,M}^{n}}  +  \tvnorm{\updelta_x R_{1/n,M}^{n} -  \updelta_y R_{1/n,M}^{n}} +  \tvnorm{\updelta_y P_1 - \updelta_y R_{1/n,M}^{n}}  \eqsp,% \\
%                                            % &\leq C_3 (1/i)^{1/2}(V(x) + V(y))  + 1 - 2\Phibf(- \alpha_*^{-1/2} \|x-y\|) \eqsp .
%   \end{equation}
%   where $R_{1/m}$ is the Markov kernel defined by \eqref{eq:kernel_langevin} with $\Tg(x) = x +\gamma b_{\gamma,M}(x)$. 
%   % We introduce the reflexion coupling $(X_k, Y_k)_{k \in \nset}$ associated to the kernel $R_{1/m}$ and starting from $(x,y)$, see \Cref{sec:quant-conv-discr} for more details\alain{vu qu'on utilise ap le couplage updater}
%   % Note that in this case, since $\msx = \rset^d$ and $\Pi = \mathrm{Id}$, $\Kcoupling_{1/m}$ is the reflection coupling associated with $(\Rcoupling_{1/m}, \Rcoupling_{1/m})$. Therefore we have for any $x, y \in \rset^d$, $n \in \nsets$
%   % \begin{equation}
%   %   \tvnorm{\updelta_x \Rcoupling_{1/m} - \updelta_y \Rcoupling_{1/m}} = \Kcoupling_{1/m}((x,y), \Delta^{\complementary}) \eqsp .
%   % \end{equation}
%   % Let $n \geq \ceil{M} \ceil{\tilde{L}_M} |m|^{-1} \1_{(-\infty,0)}(m)$. Let $\Xi_k(n) = n^{-1}\sum_{i=1}^k (1 + n^{-1}\kappa(n))^{-i}$ with $\kappa(n) = m + n^{-1}L_M$. Note that $\kappa(n) m \geq 0$. Using \Cref{theo:strict_convergence_AR}, \Cref{lemma:technical_doeb}, \Cref{ass:item:diff_disc}-\ref{item:local_lip}, \Cref{ass:item:diff_disc}-\ref{item:local_curv} we obtain that
%   Using \Cref{ass:item:diff_disc}-\ref{item:local_lip} and \Cref{ass:item:diff_disc}-\ref{item:local_curv} we have that $T_{1/m}$ satisfies \Cref{assum:lip_op}($\cball{0}{M}$). Let $N \in \nsets$ such that for any $n \geq N$, $(2\tilde{m} + n^{-1}\tilde{L}_M^2)\tilde{m} \geq  0$. In this case we obtain that for any $n \geq N$, $\kappa(1/n) < 0$ or for any $n \geq N$, $\kappa(1/n) \geq 0$. We apply \Cref{lemma:doeb} and we have that for any $x, y \in \rset^d$
%   \begin{align}
%     &\proba{X_k \neq Y_k \text{ and for any $k \in \{1,\ldots,n-1\}$,} \, (X_k,  Y_k) \in \cball{0}{M}^2} \\ & \hspace{1.5cm} \leq \1_{\Deltar^{\complem}}(x,y) \defEns{1-2\Phibf\parenthese{-\frac{\norm{x-y} }{2\Xi_n^{1/2}}}}  \leq 1 - 2\Phibf(-\alpha(n)^{-1/2}\| x- y \|) \eqsp , \label{eq:doeb_constrained} \label{eq:doeb_continuous}
%   \end{align}
%     where
%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]
%   \item $\alpha(n) = (-4/ \kappa(n)) \parentheseDeux{ \exp(-\kappa(n)) - 1}$ if $m < 0$ ; \label{item:m_neg}
% %  \item $\alpha(n,k) = 4\ell$ if $\sup_{\gamma \in \ooint{0,\bgamma}} \  m=  0$ ; \label{item:m_0}    
%   \item $\alpha(n) = (4/ \kappa(n)) \parentheseDeux{ 1 - \exp \defEns{-\kappa(n) / (1 + n^{-1}  \kappa(n))}}$ if $ m \geq 0$. \label{item:m_pos}
%   \end{enumerate}
%   Let $\alpha_{\continuous} \in \rmC(\rset,[4,+\infty))$, defined for any $t \neq 0$ by $ \alpha_{\continuous}(t) = 4t^{-1}(1 - \exp(-t))$ and $\alpha_{\continuous}(0) = 4$. We have that for any $x, y \in \rset^d$
%   \begin{equation}
%     \lim_{n \to + \infty} \proba{X_k \neq Y_k \text{ and for any $k \in \{1,\ldots,n-1\}$,} \, (X_k,  Y_k) \in \cball{0}{M}^2} \leq 1 - 2\Phibf(-\alpha_{\continuous}(\tilde{m})^{-1/2}\norm{x-y}) \eqsp . \label{eq:limite_uno}
%   \end{equation}
% Using \Cref{ass:item:diff_disc}-\ref{item:lyap_majo}, the fact that $(W(X_k)/C_2^{k(1 +n^{-\vareps}C_M)/n})_{k \in \nset}$ is a supermartingale and the maximal Doob inequality \valentin{ref}
%   \begin{align}
%     \probaMarkov{x}{\sup_{k \in \lbrace 1,  n \rbrace} \norm{X_k} > M} &\leq \probaMarkov{x}{\sup_{k \in \lbrace 1,  n \rbrace} W(X_k)/C_2^{k(1 +n^{-\vareps}C_M)/n} \geq M/ C_2^{1 +n^{-\vareps}C_M}} \\
%     &\leq C_2^{1 + n^{-\vareps}C_M}M^{-1} W(x) \eqsp . \label{eq:limite_duo} 
%   \end{align}
%   Using the fact that $(X_k,Y_k)_{k \in \nset}$ is a coupling, we obtain that
%   \begin{align}
%     \tvnorm{\updelta_xR_{1/n,M}^{n} - \updelta_yR_{1/n,M}^{n}} &\leq \proba{X_k \neq Y_k \text{ and for any $k \in \{1,\ldots,n\}$,}\, (X_k,  Y_k) \in \cball{0}{M}^2} \\ &\phantom{a} + \probaMarkov{x}{\sup_{k \in \lbrace 1, \dots, n \rbrace} \| X_k \| \geq M} + \probaMarkov{y}{\sup_{k \in \lbrace 1, \dots, n \rbrace} \| X_k \| \geq M} \eqsp . \label{eq:ineq_coupling}
%   \end{align}
%   Therefore combining \eqref{eq:limite_uno}, \eqref{eq:limite_duo} and \eqref{eq:ineq_coupling} we get that
%   \begin{equation}
%     \lim_{M \to + \infty} \lim_{n \to + \infty} \tvnorm{\updelta_xR_{1/n,M}^{n} - \updelta_yR_{1/n,M}^{n}} \leq 1 - 2 \Phibf(-\alpha_{\continuous}(\tilde{m})^{-1/2}\| x - y \|) \eqsp . \label{eq:limite_doeb1}
%   \end{equation}
%                                          Using \Cref{lemma:V-norm_control} and \eqref{eq:limite_doeb1} we obtain that for any $x,y \in \rset^d$
%                                          \begin{equation}
%                                          \tvnorm{\updelta_x P_1 - \updelta_y P_1}   \leq 1 - 2\Phibf(-\alpha_{\continuous}(\tilde{m})^{-1/2} \|x-y\|) \eqsp.     
%   \end{equation}  
% \end{proof}

Finally, we state a convergence theorem in $V$-norm for the continuous process using only regularity and one-sided conditions on $b$ as well as a continuous Foster-Lyapunov drift condition on the infinitesimal generator $\generator$.
\begin{theorem}
  \label{thm:c_contrac}
  Assume that there exist $\zeta >0 $, $B \geq 0$  a measurable function $\V\in \rmC^2(\rset^d, \coint{1,+\infty})$ such that  such that $\generator$ satisfies \hyperlink{ass:drift_continuous}{$\bfDc(V,\zeta, B)$} and $\lim_{\norm{x} \to +\infty} V(x) = +\infty$.  Assume \tup{\Cref{as:item:lip}-\ref{assum:b_min}($\mtt, \rset^d$)}, \tup{\Cref{ass:loc_lip_b}}, \tup{\Cref{ass:item:diff_disc}} and
\tup{\Cref{assum:unif_integr}}. Then there exists $C \geq 0$, $\rho \in (0,1)$ such that for any $n \geq 0$,
  \begin{equation}
    \Vnorm{\updelta_x \Pker_n - \updelta_y \Pker_n} \leq C \rho^n (V(x) + V(y)) \eqsp ,
  \end{equation}
  with
    \begin{equation}
    \begin{aligned}
         C &= (1 +  A)(1 + \left. c \middle/ \defEns{(1-\vareps)(1- \lambda)}) \right. \eqsp , \\
         \lambda &= (\exp(-\zeta) + 1)/2 \eqsp, \quad c = \exp(-\zeta) M + A \eqsp, \quad A = B(1 - \exp(-\zeta)) \eqsp, \\
         \log(\rho) &= \left. \defEns{\log(1-\vareps) \log(\lambda)} \middle/ \defEns{\log(1-\vareps) + \log(\lambda) - \log(c) } \right. \eqsp, \\
         \log(1 - \vareps) &= \log(1 - 2\Phi(-\alpha_{\continuous}(\mtt, 1)^{-1/2}R_M/2 ))\eqsp , \\
         M &= 2B/\zeta \eqsp , \quad R_M = \sup \ensemble{\norm{x-y}}{V(x) + V(y) \leq 2M} \eqsp .
      \end{aligned} 
    \end{equation}
    where $\alpha_{\continuous}$ is given in \Cref{prop:doeb_continuous}.
\end{theorem}

\begin{proof}
  Let $\Lcoupling$ be the reflection Markov kernel coupling for $\Pker_1$.
  Using \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_b}, we obtain that $\Lcoupling$ satisfies \hyperlink{ass:drift_discrete}{$\bfDd(W,\exp(-\zeta), B(1-\exp(-\zeta))/\zeta, \rset^d)$}, with $W(x,y) = (V(x) + V(y))/2$.
  Let $M = 2B/\zeta$ and define $R_M = \sup \ensemble{\norm{x-y}}{(x,y) \in \msc_M} <+\infty$, with $\msc_M = \ensemble{(x,y)}{W(x,y) \leq M}$.
  It is clear that \eqref{eq:minoration_eric_Q} with $\ell = 1$ is equivalent to $\tvnorm{\updelta_x \Pker_1 - \updelta_y \Pker_1} \leq 2(1 - \vareps)$\valentin{des deux qui trainent ?}. Using \Cref{prop:doeb_continuous} we obtain that for any $x,y \in \msc_M$
  \begin{equation}
  \tvnorm{\updelta_x \Pker_{1} - \updelta_y \Pker_{1}}   \leq 1 - 2\Phibf(-\alpha_{\continuous}(\mtt, 1)^{-1/2} R_M/2) \eqsp.
\end{equation}
Therefore, applying \Cref{thm:v_ergo_gene}, we obtain that there exist $\rho \in \ooint{0,1}$ and $C \geq 0$ such that for any $x,y \in \rset^dd$
\begin{equation}
  \Vnorm{\updelta_x \Pker_{n} - \updelta_y \Pker_{n}} \leq C \rho^n (V(x) + V(y)) \eqsp ,
\end{equation}
  with $C$ and $\rho$ given in \Cref{thm:v_ergo_gene}.
\end{proof}

% \begin{theorem}
%   \label{thm:c_contrac}
% Let $V : \rset^d \to \coint{1,\plusinfty}$ with $\lim_{\norm{x} \to \plusinfty} V(x) = \plusinfty$, $\zeta >0$ and $B \geq 0$.  Assume \Cref{ass:loc_lip_b}, \hyperlink{ass:drift_continuous}{$\bfDc(V,\zeta,B)$}, \Cref{ass:item:diff_disc} and
% \Cref{assum:unif_integr}. Then, $(P_t)_{t \geq 0}$ admits a  unique invariant probability measure and for any $x,y \in \rset^d$,
%   \begin{equation}
%     \Vnorm{\updelta_x P_t - \updelta_y P_t } \leq C \rho^t \parenthese{V(x) + V(y)} \eqsp,
%   \end{equation}
%   where
%   \begin{align}
%         C &=  (1 + B/\zeta) \rho^{-1} [1 + \exp(\zeta) B/\zeta ][1 + \left. \bc \middle/\defEns{(1-\vareps_{\continuous})(1-\lambdab)} \right.]  \eqsp, \\
%         \log(\rho) & = \left. \defEns{\log(1-\vareps_{\continuous}) \log(\lambdab) } \middle/ \defEns{\log(1- \vareps_{\continuous}) + \log(\lambdab) - \log(\bc) } < 0 \right. \eqsp, \\
%     \bc &= 3  B\exp(\zeta)/\zeta \eqsp, \quad \lambdab= (\exp(-\zeta)+1)/2 \eqsp , \quad K_{\continuous} = 2 B \exp(\zeta)/\zeta \eqsp , \quad \vareps_{\continuous} = 2 \Phibf\parenthese{- \varphi(\tilde{m})^{-1/2} M_{\continuous}} \eqsp , \\
%            M_{\continuous} &= \ceil{\sup \ensemble{ M \geq 0 }{ \text{ there exists $x,y \in \msx$ with $\norm{x-y} \leq M$}, V(x,y) \leq K_{\continuous} }} \eqsp .
%   \end{align}
% \end{theorem}

% \begin{proof}
% \Cref{prop:doeb_continuous} shows that all compact sets of $\rset^d$ are small for $P_1$. Then, since \hyperlink{ass:drift_continuous}{$\bfDc(V,\zeta,B)$} holds with $\lim_{\norm{x} \to \plusinfty} V(x) = \plusinfty$ and $\zeta >0$, the conditions of \cite[Theorem 5.1]{meyn1993criteria_iii} hold and therefore $(P_t)_{t \geq 0}$ admits a unique invariant probability measure.
%   The rest of proof is divided in two parts
%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]  
%   \item Using \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_b}, there exist $\lambda \in \ooint{0,1}$ and $A\geq0$ such that $P_1$ satisfies $\bfDd(V,\lambda, A)$ with
%     \begin{equation}
%       \lambda = \exp(-\zeta) \eqsp , \qquad A = B(1 - \exp(-\zeta))/\zeta \leq B \eqsp .
%     \end{equation}

%   \item  % We denote $\alpha_* = \inf_{\gamma \in \ooint{0, \bgamma}} \alpha(\gamma)$. Using \Cref{lemma:doeb}, \Cref{lemma:drift_c}, the fact that for any probability measure $\mu$, $\tvnorm{\mu} \leq \Vnorm[V^{1/2}]{\mu}$ and \Cref{lemma:V-norm_control} we
%     We now derive a Doeblin condition for $\delta_x P_1$. 
%   Let $M > 2A/(1-\lambda)$. Let $M_{\continuous} \in \nsets$ satisfying $\{ V \leq M \} \subset \boulefermee{0}{M_{\continuous}}$ and \Cref{prop:doeb_continuous} implies that for any $x,y \in \ball{0}{M_{\continuous}}$
%   \begin{equation}
%     \tvnorm{ \updelta_x P_1 -  \updelta_y P_1 } \leq 1- \vareps_{\continuous} \eqsp,         
%   \end{equation}
%   with $ \vareps_{\continuous} = 2 \Phibf\parenthese{- \varphi(\tilde{m})^{-1/2} M_{\continuous}}$.
%     \end{enumerate}
%   Therefore applying \Cref{theo:discrete_contrac_wass}-\ref{propo:discrete_contrac_wass_b} there exist $\rho \in \ooint{0,1}$ and $C' \geq0$ such that $P_1$ satisfies for any probability measures $\mu_0, \nu_0$ over $(\rset^d, \mcb{\rset^d})$
%   \begin{equation}
%     \Vnorm{\mu_0 P_n - \nu_0 P_n } \leq C' \rho^{n} \Vnorm{\mu_0 - \nu_0} \eqsp ,
%   \end{equation}
%   with
%   \begin{align}
%         C' &=  [1 + \lambda^{-1} A\log(1/\lambda)^{-1}][1 + \left. \bc \middle/\defEns{(1-\vareps_{\continuous})(1-\lambdab)} \right.]  \eqsp, \\
%         \log(\rho) & = \left. \defEns{\log(1-\vareps_{\continuous}) \log(\lambdab) } \middle/ \defEns{\log(1- \vareps_{\continuous}) + \log(\lambdab) - \log(\bc) } < 0 \right. \eqsp, \\
%         \bc &= 3  A\lambda^{-1} \log(\lambda^{-1})^{-1} \eqsp, \quad \lambdab= (\lambda+1)/2 \eqsp .
%   \end{align}
%   In addition, \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_b} implies that for any $t \in \ccint{0,1}$
%   \begin{equation}
%     \Vnorm{ \mu_0 P^t - \nu_0 P^t } \le (1+B/\zeta) \Vnorm{\mu_0 - \nu_0} \eqsp.
%   \end{equation}
%   Therefore we get for any $t>0$
%   \begin{align}
%     \Vnorm{\mu_0 P^t - \nu_0 P^t } &= \Vnorm{(\mu_0P^{\floor{t}} - \nu_0 P^{\floor{t}}) P^{t - \floor{t}}} \\
%                                    &\leq C' (1+B/\zeta) \rho^{\floor{t}} \Vnorm{\mu_0 - \nu_0} \leq C' (1+B/\zeta) \rho^{-1} \rho^{t} \Vnorm{\mu_0 - \nu_0} \eqsp ,
%   \end{align}
%   which concludes the proof.

% \end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> postponed_proof.tex <==
\section{Postponed Proofs}
\label{sec:postponed-proofs}

\subsection{Proof of \Cref{prop:mini_prop}}
\label{prop:mini_prop:proof}


  







% \section{Postponed Proofs}
% \label{sec:postponed-proofs}
% \subsection{Proof of \Cref{lemma:technical_doeb_0}}
% \label{sec:proof-crefl}

% Let $\ell \in \nsets$ and $\gamma \in \ocint{0,\bgamma}$. First note that the  following equalities hold if $\upkappa(\gamma) \neq 0$
%     \begin{align}
%     \Xi_{\ell \ceil{1/\gamma}}(\upkappa) &=  \gamma \sum_{i=1}^{\ell \ceil{1/\gamma}} (1+ \gamma  \upkappa(\gamma))^{-i}\\
%     &= \gamma (1 + \gamma  \upkappa(\gamma))^{-1}\frac{1 - (1+\gamma  \upkappa(\gamma))^{-\ell \ceil{1/\gamma}}} {1 - (1 + \gamma  \upkappa(\gamma))^{-1}} \\
%       &= - \upkappa^{-1}(\gamma) \defEns{\parentheseDeux{1 + \gamma  \upkappa(\gamma)}^{-\ell \step} -1} \\
%       &= - \upkappa^{-1}(\gamma) \defEns{ \exp\parentheseDeux{-\ell\ceil{1/\gamma} \log \defEns{1 + \gamma  \upkappa(\gamma)}} -1} \eqsp . \label{eq:Xi_majo_2}
%     \end{align}
%   We now give a lower-bound on $\Xi_{\ell \step}(\upkappa)$ depending on the condition satisfied by $\gamma \mapsto \upkappa(\gamma)$.
%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]
%   \item 
%     Assume that for any $\tgamma \in \ocint{0,\bgamma}$ $,  \upkappa (\tgamma) < 0$. 
%     Using that $\log(1-t) \le -t$ for $t \in \ooint{0,1}$, we obtain that
%   \begin{equation}
%     \exp\parentheseDeux{-\ell\ceil{1/\gamma} \log \defEns{1 + \gamma  \upkappa(\gamma)}} \geq \exp (-\ell\ceil{1/\gamma} \gamma  \upkappa(\gamma) ) \geq \exp(-\ell \upkappa(\gamma)) \eqsp ,
%   \end{equation}
%   which together with \eqref{eq:Xi_majo_2} concludes the proof for \ref{item:kappa_neg}.
% \item     Assume that for any $\tgamma \in \ocint{0,\bgamma}$, $  \upkappa (\tgamma) \leq 0$. Then,
%   \begin{equation}
%     \Xi_{\ell \step}(\upkappa) =  \gamma \sum_{i=1}^{\ell \ceil{1/\gamma}} (1+ \gamma  \upkappa(\gamma))^{-i} =  \gamma \step \ell \geq   \ell \eqsp .
%   \end{equation}
%   \item      Assume that for any $\tgamma \in \ocint{0,\bgamma}$ $,  \upkappa (\tgamma) >  0$. Using that $\log(1+at) /t \geq a / (1+at)$ for $t,a >0$, we obtain that
%   \begin{multline}
%     \exp\parentheseDeux{-\ell\ceil{1/\gamma} \log \defEns{1 + \gamma  \upkappa(\gamma)}} \leq \exp \parentheseDeux{-(\ell/\gamma) \log\defEns{1 + \gamma  \upkappa(\gamma)} } \\
%     \leq \exp \parentheseDeux{-\ell \upkappa(\gamma) /(1+\gamma  \upkappa(\gamma))} \eqsp ,
%   \end{multline}
%   which concludes the proof for \ref{item:kappa_pos}.
% \end{enumerate}


% \subsection{Proof of \Cref{prop:a1_type}}


%   \label{prop:a1_type:proof}
%     \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]    
%   \item By \Cref{as:item:lip} and \Cref{as:b_min}($\mtt$) we have  for any $\gamma >0$ and $x,y \in \msx$,
% $      \norm{\Tg(x) - \Tg(y)}^2 \leq (1 - 2\gamma \mtt + \gamma^2 \Lip^2) \norm{x-y}^2 \leq (1 + \gamma \kappa(\gamma)) \norm{x-y}^2$,    which concludes the proof. 
%   \item By \eqref{eq:descent_lemma}, we have for any $\gamma >0$ and $x,y \in \msx$,
% $      \norm{\Tg(x) - \Tg(y)}^2 \leq  \norm{x-y}^2 + \gamma(-2\Lipb + \gamma)\norm{b(x) - b(y)}^2$.    Then if $\gamma \leq 2 \Lipb$, $      \norm{\Tg(x) - \Tg(y)}^2 \leq  \norm{x-y}^2$, which concludes the proof.
%   \end{enumerate}


% \subsection{Proof of \Cref{propo:drift_strong_convex}}
%   \label{propo:drift_strong_convex:proof}


%     Let $\gamma \in \ocint{0, \bgamma}$ and $x \in \msx$. Using \eqref{eq:langevin_discrete}, \Cref{as:item:lip}, \Cref{as:b_min}($\mtt$), \Cref{assum:drift_strong} and that the projection $\Pi_{\msx}$ is non expansive we obtain the following inequalities
%   \begin{align}
%     \Rcoupling_{\gamma}V(x)
%                               &\leq 1 + \norm{x + \gamma b(x)}^2 + \gamma d \\
%                      &\leq1 + \norm{x}^2 + 2\gamma \langle x, b(x) \rangle + \gamma^2 \norm{b(x)}^2 + \gamma d \\
%     &\leq (1 + \norm{x}^2) \parentheseDeux{1 - \gamma(2\mttplusdeux - \bgamma \Lip^2)} + \gamma \parenthese{d + 2\Rdeux^2(\mttplusdeux - \mtt)_+ + 2\mttplusdeux} \eqsp ,
%   \end{align}
% which concludes the proof using \Cref{lemma:drift_2_drift_1}.

% \subsection{Proof of \Cref{propo:drift_strong_convex_bounds}}
%   \label{propo:drift_strong_convex_bounds:proof}  
%   Let $\bgamma \in \ooint{0, 2\mttplus / \Lip^2}$. Using \Cref{propo:drift_strong_convex} we obtain that for any $\gamma \in \ocint{0, \bgamma}$, $\Kcoupling_{\gamma}$ satisfies \hyperlink{ass:drift_discrete}{$\bfDd(W,\lambda^{\gamma},A \gamma, \msx)$}, with $\lambda$ and $A$ explicitly given by in \Cref{propo:drift_strong_convex}.
%   For any $x,y \in \msx$ such that $\norm{x-y} \geq M_{\discrete}$, either $V(x) \geq 2 \Bdisc$ or $V(y) \geq 2 \Bdisc$, and therefore $W(x,y) > \Bdisc$. Note also that \eqref{eq:minorization_condition_v2} is satisfied for any $\gamma \in \ocint{0, \bgamma}$ and $x,y \in \msx$  and \Cref{theo:minorization_general} and \Cref{lemma:technical_doeb_0}. Therefore we can apply \Cref{theo:discrete_contrac_wass}, which concludes the proof.  

% \subsection{Proof of \Cref{propo:drift_convex}}
% \label{propo:drift_convex:proof}


%    Let $\gamma \in \ocint{0, \bgamma}$. Using the fact that $\Pi_{\msx}$ is non expansive, the Log-Sobolev inequality \cite[Theorem 5.5]{boucheron2013concentration} and the Jensen inequality we obtain for any $x \in \rset^d$
%    \begin{align}
%      \Rker_{\gamma} V(x) &\leq \exp \parentheseDeux{\mtttrois \Rker_{\gamma}\phi(x) + \gamma (\mtttrois)^2/2} \leq \exp \parentheseDeux{\mtttrois \sqrt{1 + \Rker_{\gamma}\norm{x}^2} + \gamma (\mtttrois)^2/2 } \\ &\leq  \exp \parentheseDeux{\mtttrois \sqrt{1 + \norm{\Tg(x)}^2 + \gamma d} + \gamma (\mtttrois)^2/2 } \eqsp . \label{eq:ineq_1_curv}
%    \end{align}
%    Let $x \in \rset^d$. The rest of the proof is divided in two parts.
%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]
%   \item    
%    In the first case, $\norm{x} \geq \Rquatre$.
% Since $\norm{x} \geq \Rtrois$ and $\gamma \leq 2\mttdeux$, we have using \tup{\Cref{assum:curvature}}
% \begin{equation}
%   \norm{\Tg(x)}^2 \leq \norm{x}^2 - 2\gamma \mttun  \norm{x} + \gamma(\gamma - 2\mttdeux) \norm{b(x)}^2 + \gamma c \leq \norm{x}^2 - 2\gamma \mttun \norm{x} + \gamma c \eqsp . \label{eq:ineq_2_curv}
% \end{equation}
% Since $\norm{x} \geq 1$ we have $2 \norm{x} \geq \phi(x)$ and therefore, using that $\norm{x} \geq (d+c)/\mttun$, $2 \mttun \norm{x} \geq 2 \mtttrois \phi(x) + d +c$. This inequality, combined with the fact that for any $t \in \ooint{-1,+\infty}$, $\sqrt{1 + t} \leq 1 + t/2$, yields
% \begin{equation}
%   \sqrt{1 + \norm{x}^2 + \gamma (-2\mttun \norm{x} + d +c)} - \phi(x) \leq \gamma (-2 \mttun \norm{x} + d+c)/(2\phi(x)) \leq - \mtttrois \gamma \eqsp . \label{eq:ineq_3_curv}
% \end{equation}
% Combining \eqref{eq:ineq_1_curv}, \eqref{eq:ineq_2_curv} and \eqref{eq:ineq_3_curv} we get
% \begin{equation}
%   \Rker_{\gamma} V(x) \leq \lambda^{\gamma} V(x) \eqsp .
% \end{equation}
% \item In the second case $\norm{x} \leq \Rquatre$. We have the following inequality using \tup{\Cref{assum:curvature}} and that $\gamma \leq 2 \mttdeux$
%   \begin{equation}
%     \norm{\Tg(x)}^2 \leq \norm{x}^2  + \gamma(\gamma - 2\mttdeux) \norm{b(x)}^2 + \gamma c \leq \norm{x}^2  + \gamma c \eqsp . \label{eq:ineq_4_curv}
%   \end{equation}
%  Combining \eqref{eq:ineq_1_curv}, \eqref{eq:ineq_4_curv} and the fact that for any $t \in \ooint{-1,+\infty}$, $\sqrt{1 + t} \leq 1 + t/2$ we get
%  \begin{equation}
%    \Rker_{\gamma} V(x) \leq \exp \parentheseDeux{ \gamma \mtttrois (d+c)/(2\phi(x)) + \gamma (\mtttrois)^2/2 }V(x) \leq \exp\parentheseDeux{\gamma (\mtttrois (d+c) + (\mtttrois)^2)/2}V(x) \eqsp . \label{eq:ineq_5_curv}
%  \end{equation}
% Note that for any $c_1 \geq c_2$ and $t \in \ccintLigne{0, \bar{t}}$  we have the following inequality
% \begin{equation}
%   \rme^{c_1 t} \leq \rme^{c_2 t} + \rme^{c_1 \bar{t}}(c_1 - c_2)t \eqsp . \label{eq:ineq_6_curv}
% \end{equation}
% Combining \eqref{eq:ineq_5_curv} and \eqref{eq:ineq_6_curv} we get
% \begin{equation}
% \Rker_{\gamma} V(x) \leq \lambda^{\gamma}V(x) + \exp\parentheseDeux{\bgamma (\mtttrois (d+c) + (\mtttrois)^2)/2}(\mtttrois (d+c)/2 + (\mtttrois)^2)\exp(\mtttrois (1 + \Rquatre^2)^{1/2})\gamma \eqsp ,
% \end{equation}
% which concludes the proof.
%   \end{enumerate}



% \subsection{Proof of \Cref{propo:weak_outside_bounds}}
% \label{propo:weak_outside_bounds:proof}

%   Let $\bgamma \in \ocint{0, 2 \mttdeux}$. Using \Cref{propo:drift_strong_convex} we obtain that for any $\gamma \in \ocint{0, \bgamma}$, $\Kcoupling_{\gamma}$ satisfies \hyperlink{ass:drift_discrete}{$\bfDd(W,\lambda^{\gamma},A \gamma, \msx)$}, with $\lambda$ and $A$ explicitly given in \Cref{propo:drift_strong_convex}. Let 
%   \begin{equation}\Bdisc = 2 A (1 + \bgamma)(1 + \log^{-1}(1/\lambda)) \quad \text{and} \ M_{\discrete} =  2\log(2\Bdisc)/\mtttrois\eqsp.
%   \end{equation}
%   Note that for any $x,y \in \msx$ such that $\norm{x-y} \geq M_{\discrete}$, either $V(x) \geq 2\Bdisc$ or $V(y) \geq 2\Bdisc$, and therefore $W(x,y) > \Bdisc$. The rest of the proof is similar to the one of  \Cref{propo:drift_strong_convex_bounds}.

% \subsection{Proof of \Cref{prop:existence_integr}}
% \label{prop:existence_integr:proof}

%   Let $p \in \nsets$ and $V \in \rmC^2(\rset^d, \coint{1,+\infty})$ be defined for any $x \in \rset^d$ by $V(x) = 1 + \norm{x}^{2p}$.
%   We have that $\nabla V(x) = 2p \norm{x}^{2(p-1)}x$ and $\Delta V(x) = (4p(p-1) + 2pd)\norm{x}^{2(p-1)}$. Therefore, using \Cref{as:b_min}($\mtt$) 
%   and the definition of $\generator$
%   we obtain that for any $x \in \rset^d$
%   \begin{equation}
%     \generator V(x) \leq \parentheseDeux{2p(p-1) + p(d - 2\mtt)}V(x) \eqsp . \label{eq:drift_1}
%   \end{equation}
%   Hence, using \eqref{eq:drift_1} and \cite[Theorem 3.5]{khasminskii2011stochastic}, we obtain that $(\bfX_t)_{t \geq 0}$ is defined for any $t \geq 0$, for any starting point $\bfX_0 = x\in \rset^d$. In addition, we have:
%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]    
%   \item if there exists $\vareps_b >0$ such that $\sup_{x \in \rset^d} \norm{b(x)}^{2(1+\vareps_b)}(1 + \norm{x}^{2p})^{-1} < +\infty$, using \eqref{eq:drift_1} and \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_a} we obtain that \Cref{assum:unif_integr} holds.
%   \item if there exists $\vareps_b >0$ such that $\sup_{x \in \rset^d} \norm{b(x)}\rme^{-\mttplusdeux\norm{x}^2} < +\infty$, and 
%     \Cref{assum:drift_strong} holds, then we set $V \in \rmC^2(\rset^d, \coint{1,+\infty})$ where for any $x \in \rset^d$, $V(x) = \rme^{\mttplusdeux \norm{x}^2}$. We have the following inequalities for any $x \in \cball{0}{\Rdeux}^{\complementary}$,
%     \begin{equation}
%       \generator V(x) \leq \mttplusdeux\parentheseDeux{d + (2\mttplusdeux - 4\mttplusdeux/2)\norm{x}^2}V(x) \leq \mttplusdeux d V(x) \eqsp . \label{eq:drift_2}
%     \end{equation}
%     Setting $\zeta = (\mttplusdeux d) \vee \sup_{x \in \cball{0}{\Rdeux}} \generator V(x)$, we obtain that $V$ satisfies \hyperlink{ass:drift_continuous}{$\bfDc(V,\zeta,0)$}. Therefore using \eqref{eq:drift_2} and \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_a}
%     , we obtain that \Cref{assum:unif_integr} holds.
%   \end{enumerate}

% \subsection{Proof of \Cref{prop:fam_prop}}
% \label{prop:fam_prop:proof}

%   \begin{enumerate}[label= (\alph*),  wide, labelwidth=!, labelindent=0pt]    
%   \item It is easy to check that \Cref{ass:diff_disc} holds with $\beta = 2\alpha$. \Cref{ass:seq_k_n} is trivial. It only remains to show that \Cref{ass:lyap_majo} holds. Let $W(x) = \norm{x}$, $n \in \nset$, $\gamma \in \ocint{0, \bgamma}$, $x \in \rset^d$ and $X = x + \gamma b_{\gamma, n}(x) + \sqrt{\gamma} Z$, where $Z$ is a $d$-dimensional Gaussian random variable with zero mean and covariance identity. We have the following inequality using \Cref{as:b_min}($\mtt$)
%   \begin{equation}
%     \expe{\norm{X}^2} \leq  \|x \|^2 - 2 \gamma  \mtt_0 \Phi_n(x) \norm{x}^2 + \gamma^2 \Phi_n(x)^2 \norm{b(x)}^2 +  \gamma d  \eqsp , \label{eq:numero_uno}
%   \end{equation}
%   with $\Phi_n(x) = \varphi_n(x) + (1 - \varphi_n(x))(1 + \gamma^{\alpha}\norm{b(x)})^{-1}\leq 1$. We also have that for any $n \in \nset$ and $x \in \rset^d$
%   \begin{equation}
%     \Phi_n(x) \norm{b(x)} \leq \Lip_{n+1}\norm{x}  + \gamma^{-\alpha} \eqsp . \label{eq:numero_duo}
%   \end{equation}
% Combining \eqref{eq:numero_uno} and \eqref{eq:numero_duo} we obtain
% \begin{equation}
%   \expe{1 + \norm{X}^2} \leq (1 + \norm{x}^2)\parentheseDeux{1 -  2 \gamma \mtt_0 + 2 \gamma^2 \Lip_{n+1}^2} + 2 \gamma^{2 - 2\alpha} + \gamma d \eqsp , \label{eq:control_norm_2}
% \end{equation}
% which concludes the proof of \Cref{prop:fam_prop}-\ref{prop:fam_prop_a} upon taking $\tilde{A} = \exp(2 \abs{\mtt} + d + 1)$, $\varepsn = 1 - 2\alpha$ and $\En = 2(\Lip_{n+1} \bgamma^{2\alpha} + 1)$.
% \item
% Let $n \in \nset$. Using the Log-Sobolev inequality \cite[Theorem 5.5]{boucheron2013concentration}, the fact that $\Pi_{\msk_n}$ is non expansive  and the Jensen inequality we obtain for any $\gamma \in \ocint{0, \bgamma}$ and $x \in \rset^d$,
%      \begin{equation}
%      \Rker_{\gamma} V(x) \leq \exp \parentheseDeux{ \Rker_{\gamma}\phi(x) + \gamma ^2/2} \leq \exp \parentheseDeux{ \sqrt{ \Rker_{\gamma}(1+\norm{x}^2)} + \gamma ^2/2 } \eqsp .\label{eq:log_sob}
%    \end{equation}
%    We have that $\sup_{x \in \rset^d} \Phi_n(x) \norm{b(x)} \leq (\sup_{x \in \cball{0}{n+1}} \norm{b(x)}\bgamma^{\alpha} +1)\gamma^{-\alpha}$. Let $B_n = \sup_{x \in \cball{0}{n+1}} \norm{b(x)}$.
%   Using \eqref{eq:numero_uno} and  \Cref{assum:drift_strong}, we obtain that for any $\gamma \in \ocint{0, \bgamma}$ and $x \in \cball{0}{\Rdeux}^{\complementary}$,
%   \begin{equation}
%     \Rker_{\gamma}(1 + \norm{x}^2) \leq 1 + \norm{x}^2\parentheseDeux{1 -  2 \gamma \mttplusdeux\Phi_n(x) } + \gamma^{2(1-\alpha)} \parenthese{1 + \bgamma^{\alpha} B_n}^2 + \gamma d \eqsp . \label{eq:exp_1}
%   \end{equation}
% On the other hand, using \eqref{eq:control_norm_2}, we get for any $\gamma \in \ocint{0, \bgamma}$ and $x \in \cball{0}{\Rdeux}$, 
% \begin{align}
%   \Rker_{\gamma}(1 + \norm{x}^2) &\leq (1 + \norm{x}^2) + 2(\gamma |\mtt| + \gamma^2 \Lip_{n+1}^2)(1 + \Rdeux^2) + 2 \gamma^{2 - 2\alpha} + \gamma d \eqsp . \label{eq:exp_2}
% \end{align}
% Therefore, setting $\tilde{A} = \exp(d + |\mtt|(1 + R^2) + 1)$, $\varepsn = 1 - 2\alpha$ and $\En = (1 +\bgamma^{\alpha} B_n)^2/2 + \Lip_{n+1}^2(1+\Rdeux^2)\bgamma^{2\alpha} + 3/2$ and combining \eqref{eq:log_sob}, \eqref{eq:exp_1} and \eqref{eq:exp_2} with the fact that for any $t \in \ooint{-1,+\infty}$, $\sqrt{1 + t} \leq 1 +t/2$, we get for any $\gamma \in \ocint{0, \bgamma}$ and $x \in \rset^d$
% \begin{equation}
%   \Rker_{\gamma} V(x) \leq \exp \parentheseDeux{\log(C_3)\gamma (1 + \En\gamma^{\varepsn})} V(x) \eqsp. \label{eq:drift_n}
% \end{equation}
% Setting $\gamma = \Time/m$ with $m \in \nsets$, iterating \eqref{eq:drift_n} and taking the limit when $m \to +\infty$ concludes for \Cref{prop:fam_prop}-\ref{prop:fam_prop_b}.
% \end{enumerate}

% \subsection{Proof of \Cref{propo:majo_cont}}
% \label{propo:majo_cont:proof}
%   We have for any $x \in \rset^d$,
%   \begin{equation}
%     \nabla \phi(x) = x /\phi(x) \eqsp , \qquad \nabla^2 \phi(x) = \Id/\phi(x) - x x^{\transpose} / \phi(x)^2 \eqsp .
%   \end{equation}
%   In addition, for any $x \in \rset^d$,
%   \begin{equation}
%     \nabla V(x) = M \nabla \phi(x) V(x) \eqsp, \qquad \nabla^2 V(x) = \parenthese{M^2 \nabla \phi(x) (\nabla \phi(x))^{\transpose} + M \nabla^2 \phi(x)} V(x) \eqsp .
%   \end{equation}
%   Therefore, for any $x \in \rset^d$,
%   \begin{equation}
%     (\generator V(x))/V(x) \leq \parentheseDeux{M^2 \norm{x}^2/\phi(x)^2 + M(d / \phi(x) - \norm{x}^2/\phi(x)^2)}/2 + M \sup_{x \in \rset^d} \langle b(x), x \rangle \eqsp .
%   \end{equation}
%   Hence, for any $x \in \rset^d$, $\generator V(x) \leq \zeta V(x)$ with $\zeta = M(\sup_{x \in \rset^d} \langle b(x), x \rangle +d/2) + M^2$. We conclude using \Cref{lemma:disclyapfromc}-\ref{lemma:disclyapfromc_a} and the Doob maximal inequality.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

